The Seiberg-Witten Equations on Manifolds with Boundary I: The Space of Monopoles and Their Boundary Values

In this paper, we study the Seiberg-Witten equations on a compact 3-manifold with boundary. Solutions to these equations are called monopoles. Under some simple topological assumptions, we show that the solution space of all monopoles is a Banach manifold in suitable function space topologies. We then prove that the restriction of the space of monopoles to the boundary is a submersion onto a Lagrangian submanifold of the space of connections and spinors on the boundary. Both these spaces are infinite dimensional, even modulo gauge, since no boundary conditions are specified for the Seiberg-Witten equations on the 3-manifold. We study the analytic properties of these monopole spaces with an eye towards developing a monopole Floer theory for 3-manifolds with boundary, which we pursue in Part II.

==> packages.tex <==
%auto-ignore

\usepackage{amssymb, amsmath, euscript, verbatim, theorem, xr, sw,default,title,mathrsfs,array,xypic, graphicx, url, tabularx}
\usepackage[margin=32pt,font=footnotesize]{caption}
\renewcommand{\theenumi}{(\roman{enumi})}
\renewcommand{\labelenumi}{\theenumi}
\DeclareOption{ctagsplt}


